Keeping Context In Mind: Automating Mobile App Access Control with User Interface Inspection

Recent studies observe that app foreground is the most striking component that influences the access control decisions in mobile platform, as users tend to deny permission requests lacking visible evidence. However, none of the existing permission models provides a systematic approach that can automatically answer the question: Is the resource access indicated by app foreground? In this work, we present the design, implementation, and evaluation of COSMOS, a context-aware mediation system that bridges the semantic gap between foreground interaction and background access, in order to protect system integrity and user privacy. Specifically, COSMOS learns from a large set of apps with similar functionalities and user interfaces to construct generic models that detect the outliers at runtime. It can be further customized to satisfy specific user privacy preference by continuously evolving with user decisions. Experiments show that COSMOS achieves both high precision and high recall in detecting malicious requests. We also demonstrate the effectiveness of COSMOS in capturing specific user preferences using the decisions collected from 24 users and illustrate that COSMOS can be easily deployed on smartphones as a real-time guard with a very low performance overhead.

==> discussion.tex <==
%\vspace{-3ex}
 \begin{minipage}{\textwidth}
  \begin{minipage}[htb]{0.5\textwidth}
    \centering
    %\caption{\label{tab:feature}Classification with Different Feature Sets}
        \includegraphics[height=2.0in]{who.pdf}

      \captionof{figure}{Advertisement in a Weather App.
	The advertisement widget located at the bottom may stealthily collect user location by exploiting the location permission granted to the weather functionality. }\label{fig:who}
   
  \end{minipage}
  \hfill
  \begin{minipage}[htb]{0.45\textwidth}
    \centering
        \captionof{table}{Features in the  \textit{who} set}\label{tab:attributes}
\small{
\begin{tabular}{ l r }
\toprule

Feature & Description \\\midrule
%\hline
{\tt text} & The text shown on the widget\\
{\tt class} & The Java class of the widget instance\\
{\tt position} & Its relative position in the layout \\ %, which is mapped to the grids.\\
{\tt size} & The percentage of screen area occupied \\
{\tt isPassword:} & Whether the widget is a password\\
{\tt isClickable}  & Whether the widget can be clicked \\
{\tt isLongClickable} & Whether the widget can be long clicked\\
{\tt isCheckable} & Whether the widget can be checked \\
{\tt isScrollable} & Whether the widget can be scrolled\\
\bottomrule
\end{tabular}
}

    \end{minipage}
  \end{minipage}
 
\ignore{
\begin{figure}[htb]
	\centering
	\includegraphics[height=2.0in,width=0.42\textwidth]{who.pdf}
	\caption{Advertisement in a Weather App.
	The advertisement widget located at the bottom may stealthily collect user location by exploiting the location permission granted to the weather functionality.}
	\label{fig:who}
\end{figure}




\begin{table}[htb]
\begin{threeparttable}
\caption{\label{tab:attributes} }
%\small{
\begin{tabular}{ l r }
\toprule

Feature & Description \\\midrule
%\hline
{\tt text} & The text shown on the widget\\
{\tt class} & The Java class of the widget instance\\
{\tt position} & Its relative position in the layout \\ %, which is mapped to the grids.\\
{\tt size} & The percentage of screen area occupied \\
{\tt isPassword:} & Whether the widget is a password\\
{\tt isClickable}  & Whether the widget can be clicked \\
{\tt isLongClickable} & Whether the widget can be long clicked\\
{\tt isCheckable} & Whether the widget can be checked \\
{\tt isScrollable} & Whether the widget can be scrolled\\
\bottomrule
\end{tabular}

\end{threeparttable}
\end{table}
}

\ignore{  
\subsection*{Discussion on Online Permission System}
We briefly discuss how COSMOS handle corner cases related to online permission system.\\
\noindent \textbf{Background Services}
In an Android app, an {\tt Activity} can start a background {\tt Service} through inter-component communication. When a sensitive call is initiated by a {\tt Service}, its call stack does not contain the information of the starting {\tt Activity}.
In this case, {\tt COSMOS} monitors the calls of {\tt Activity.startService(Intent)} to track the relationship between running {\tt Activities} and {\tt Services}.
{\tt COSMOS} can then use the information available from the {\tt Activity} to infer the purpose of a {\tt Service} request.
%As we show later in Section~\ref{}, nearly all functionalities fulfilled by sensitive permissions involve foreground user interactions.
%However, it is possible that a legitimate sensitive method call is triggered without proper UI shown at the foreground.

One problem with this approach is that a {\tt Service} may still be alive even when the foreground {\tt Activity} has finished. In this case, {\tt COSMOS} simply notifies the user about the background request and lets the user decide whether to allow or deny the request.
Alternatively, we can always reject such requests.
We argue that sensitive services should not exist unless they provide sufficient foreground clues to indicate their purposes.
Users tend to reject requests without foreground as suggested by three recent important user studies~\cite{wagner2015, wagner2017, smarper}.
Google also further restricts background services in the most recent Android O~\cite{androido}.

\noindent \textbf{Handling of False Automatic Decisions}
Achieving 100\% precision and recall is intractable for any machine learning algorithm.
To provide better usability, COSMOS notifies the user of each rejection and provides rich contextual information, including the activation
event, the triggering widget, and the screenshot, to help the user perceive the cause.
For any false automatic decision made by the system, the user can override it at the backend and our incremental learning models will incorporate the user's decision immediately.
}

\input{rq3}

\subsection*{Discussion on Future Exploration}\label{sec:discussion}
%In this section, we discuss the limitations of our approach and make suggestions on future directions.\\
\noindent \textbf{Features} %Piggyback Attack}
We envision that it is a long-term battle to fight against increasingly more advanced adversary.
Similar to existing machine learning based detection methods~\cite{zhang2014semantics,arp2014drebin,yangappcontext,ubicomp2015,gorla2014checking,qu2014autocog}, {\tt COSMOS} could be bypassed with feature engineering through carefully designed evasion logic.
%An adversary may deliberately make an app (or repackage an existing app) that contains some valid user interfaces to justify certain permission requests while piggybacking illegitimate sensitive information flows in the same context.
%For example, he can modify an SMS app to send out user intended SMS, while at the same time, deliver messages to a malicious receiver.
However, we argue that the design philosophy of {\tt COSMOS} makes such attacks more difficult to succeed. First, the adversary can only target apps that are legitimate to use the target permissions.
%For example, he could only manipulate a limited number of communication or utility apps to access SMS related permissions.
Second, the adversary is restricted to exploit the target permissions under proper scenes only.
%For example, even if he successfully elicited an end user to install the malicious SMS app, he could only send out a message under the composing page, and when to access such pages is fully controlled by the user.
%Existing detection approaches check description-to-permission fidelity.
Thus, by enforcing contextual integrity, {\tt COSMOS} is more robust than approaches that only check description-to-permission fidelity~\cite{pandita2013whyper,gorla2014checking,qu2014autocog}.
%the adversary may not be able to bypass our defense by simply avoiding one or two features;
Third, as {\tt COSMOS} examines both the trigger events and the activation widgets, the adversary should carefully plug the payload into the correct position of the targeted app source code.
%In the example above, he cannot simply introduce a malicious background service. Instead, he should place the malicious logic inside the clicking handler of the {\tt send} button to succeed.
%needs to consider the identification power from the combination of multiple features to carefully come up with a strategy to cheat our classifier.
Moreover, {\tt COSMOS} can be integrated with other techniques based upon different feature sets to provide more comprehensive protection.
%A promising direction is to add runtime data-flow tracking support, which enables COSMOS to better understand the semantic relationships among the widgets.
%In that case, an SMS is restricted to the recipient specified by the {\tt To:} widget.
%even when the features selected for our implementation become less differentiating in the presence of a new attack, , further raising the bar to the evasion attempts.
%Therefore,
%We envision that more features need to be considered in the future, such as the interval between the requests and the SMS receiver number.

\ignore{
Although COSMOS provides a more detailed characterization of user interface than existing approaches~\cite{flowintent, backstage, asdroid, peruim} to better detect improper permission requests, it leaves room to consider more advanced features.
Moreover, an adversary who knows the precise list of features we use can potentially obfuscate the user interface to match our criteria. For example, one may put human invisible text labels (e.g. using white text on a white background) on the screen to deceive our system. %that the user is under the indicated context.
%However, such an attack can be difficult to conduct even for the current version of COSMOS. While COSMOS perceives the invisible texts, it also reads other elements visible to users that has inconsistent information.
Although such an attack is possible, it cannot easily bypass the current version of COSMOS, as COSMOS considers multiple types of UI features.
As we mentioned before, our system would warn the user if it encounters confused scenarios that do not lead to a confident decision.
%Also, it certainly leaves room to consider more.
%Future research is definitely desired to better
}

%We envision that it is a long-term battle to fight against increasingly more advanced adversary. %and when desired, we can definitely consider more UI-related features (e.g. color and images) and adapt our models for emerging new attacks.
%Our approach is flexible to incorporate more orthogonal features to cope with emerging new attacks.
%Although current COSMOS considers UI-related features as complete as possible,


\noindent \textbf{Implementation}
As mentioned in Section~\ref{sec:online}, our run-time system stores the references of encountered UI elements and leverages the information available in the call stack to match sensitive API calls to the corresponding UI elements.
However, the mapping could be imprecise due to multi-threading.
One reason is that the call stack does not contain the caller's information of a child thread.
%Although we can track the initiation procedure of certain threads, there is no universal solution yet to track all possible threads inside Android apps.
%Even if the call stack contains the caller's information, we may still incorrectly identify the relationship between sensitive calls and UI elements. % Another reason is
%For example, a user may click two buttons in a short time period, where only the first click leads to a sensitive call, but the time of actual invocation is later than the second click.
%From the call stack, we can only know that the API call was initiated by a click handler
%In this case, our current implementation matches the API call to the most recently used button, which may not be the one that triggers the sensitive call.
The problem could be alleviated by modifying the base code of {\tt Xposed} to log the values we need inside the runtime environment.

%We currently focus on the apps designed in English. However, our design could be easily extended to add multi-language support. % analyze text in other languages.
%and our tool currently cannot analyze text in other languages.
%We plan to add multi-language support in the future.

\noindent \textbf{Beyond Lab-based User Study}
%Due to the limited resources we have,
We so far did preliminary lab-based user study in evaluating our proof-of-concept system.
The demographic distribution of participants is not comprehensive and the data set is small.
Once our system is ready for daily use, we will release it to popular app stores and get feedback from actual deployments beyond the controlled lab environment.


==> rq3.tex <==
\begin{table*}[htb]
\centering
%\setlength\tabcolsep{0pt}
\begin{threeparttable}
\caption{\label{tab:thread} }
%\small{
\begin{tabular}{ l c c c c }
\toprule

Target App & Requests/min & \tabincell{c}{Time/Request(ms)} & \tabincell{c}{CPU Time/Request(ms)} & \tabincell{c}{CPU Time (\%)} \\\midrule
%\hline
\tabincell{c}{Wechat} & 12.6 & 174.7 & 76.7 & 4.4\% \\
\tabincell{c}{Yelp} & 5.8 & 56.4 & 21.8 & 2.2\% \\
Yahoo Weather & 2.5 & 42.3 & 11.3 & 1.4\% \\
\tabincell{c}{Amazon} & 0.8 & 23.0 & 8.7 & 0.6\% \\
\tabincell{c}{Paypal} & 0.4 & 27 & 11.8 & 0.2\% \\
%\tabincell{c}{Instagram} &  &  &  &  &  &  \\
%363527 & 40719 & 20 & 1936 & 1794 & 4.4\% \\
\bottomrule
\end{tabular}
%}
\end{threeparttable}
\end{table*}


\subsection*{Performance on Real Devices and Case Studies}
In this subsection, we measured the overhead incurred by {\tt COSMOS}.
We installed the online module of {\tt COSMOS} on a Google Nexus 5 running Android 5.1.1 with 2.26 GHz quad-core CPU and 2GB RAM.


\noindent \textbf{CPU Time}
We installed some popular apps from different categories on the phone, interacted with them as in common daily use, and monitored the performance overhead introduced by {\tt COSMOS}.
The performance data were collected using the runtime profiling tool Traceview~\cite{traceview}, which is officially supported for debugging Android apps through tracking the performance of each method call.
We modified the device firmware to let {\tt Traceview} monitor the released commercial apps without requiring their debuggable installation packages.
%Since INSPIRED intercepts the method calls of the target app,
The overhead introduced by {\tt COSMOS} is measured within the target monitored app. %measured with inpectation

Table~\ref{tab:thread} shows the measured CPU overhead of {\tt COSMOS} when interacting with 5 representative apps installed on the phone. Each of these apps has at least 10 million installations according to Google Play.
%The word ``incl'' is the abbreviation of ``inclusive'', means the total time
%The duration column presents the total time (ms) spent on interacting with the app.
%We did not count the time of waiting useision, which varies widely for different users.
%We only count the total time spent on actual using CPU, excluding the waiting time on I/O and the time waiting for user's decisions, which varies widely for different users.
%Inclusive time is the sum of the time spent in the methods defined by INSPIRED, as well as the sum of the times of all methods that INSPIRED call.
The first column gives the average number of sensitive requests made by each app per minute. The second column shows the average total time that {\tt COSMOS} spent on inspecting a request, excluding the time waiting for user's decisions. The third column gives the average CPU time that INSPIRED spent on a request, excluding the waiting time on I/O. The last column gives the percentage of the CPU time used by {\tt COSMOS} within an app over the total CPU time that app used during execution. Note that the value was measured within each target app, not the total CPU time used by the entire device.

We observe that {\tt COSMOS} consumed less than 5\% total CPU time for all the five apps and the values vary a lot across apps. In particular, {\tt COSMOS} incurred the highest overhead on Wechat, which can be explained by two main reasons.
First, Wechat intensively requests permissions when used.
As a complicated communication and social app, it needs to access several sensors to provide functionalities such as voice input, location sharing, video call, etc.
It also periodically reads the device ID for analytical purpose.
Second, Wechat adopts its own GUI library, which takes {\tt COSMOS} longer time for analysis.
Yelp and Yahoo Weather also frequently initiate sensitive requests.
They continuously update locations to provide nearby services and weather information, respectively.
Compared to Wechat, their UI structures are simpler. % and hence cost less time to analyze.
Amazon asks to access microphone and location for embedded voice assistance, which has limited foreground information %content information shown on the window
and was triggered only after proper user interactions.
During the experiment, Paypal only initiated sensitive requests when the app was first started.
The lower frequency of permission requests and the simpler UI together led to the least overhead for Amazon and Paypal.

%The Android virtual machine has not yet supported to measure the size of a specific memory object at runtime.
\noindent \textbf{Memory Usage}
As the method profiling provided by {\tt TraceView} did not include the memory cost.
We estimated the rough memory usage of {\tt COSMOS} by dumping the runtime objects into files. We serialized the running {\tt COSMOS} objects and the related referenced objects such as {\tt Weka} instances at the decision points, in which the memory use should reach the peak value. The average memory use was 5,712 KB over 50 separate decision points. Among them, over 95\% memory can be attributed to the {\tt Weka} machine learning module.

\noindent \textbf{Storage}
The size of the installation package of our run-time control system is 8.7 MB.
After installation, the total storage occupied is 19.86 MB, including the {\tt COSMOS} classes, {\tt Xposed} library, {\tt Weka} library, Android support library and the resource files.
We can reduce the size by discarding the unused classes files inside the libraries, and further reduction is possible by compressing some resource files.

\noindent \textbf{Network bandwidth}
{\tt COSMOS} does not generate any network traffic on its normal use. This is a significant overhead reduction compared to cloud-based systems that continuously consume bandwidth to upload user data. % for security and privacy analysis.
%INSPIRED may need the network for updating to the latest version.

